DRAMDig: A Knowledge-assisted Tool to Uncover DRAM Address Mapping

As recently emerged rowhammer exploits require undocumented DRAM address mapping, we propose a generic knowledge-assisted tool, DRAMDig, which takes domain knowledge into consideration to efficiently and deterministically uncover the DRAM address mappings on any Intel-based machines. We test DRAMDig on a number of machines with different combinations of DRAM chips and microarchitectures ranging from Intel Sandy Bridge to Coffee Lake. Comparing to previous works, DRAMDig deterministically reverse-engineered DRAM address mappings on all the test machines with only 7.8 minutes on average. Based on the uncovered mappings, we perform double-sided rowhammer tests and the results show that DRAMDig induced significantly more bit flips than previous works, justifying the correctness of the uncovered DRAM address mappings.

==> related.tex <==
\section{Related Work}\label{sec:related}
In this section, we compare our system to the existing rowhammer attacks and discuss the related defenses. 

\subsection{Rowhammer Attacks}

\eat{
\emph{\textbf{Process Isolation.}} Seaborn et al.~\cite{seaborn2015exploiting} use x86 \emph{clflush} instruction and memory spraying to escape the Native Client sandbox within a browser. Similarly, Gruss et al.~\cite{gruss2016rowhammer} crafts special memory access pattern to escape Linux scripting environment and Bosman et al.~\cite{bosman2016dedup} reply on \emph{page-deduplication}~\cite{pagededuplication} to compromise Windows-based JavaScript isolation. 
    Bhattacharya et al.~\cite{bhattacharya2016curious} utilize \emph{pagemap}~\cite{shutemovpagemap} to cause bit-flips in a running exponentiation algorithm and thus recover a secret key. Gruss et al.~\cite{gruss2017another} exploit \emph{page cache}~\cite{pagecache} to flip opcodes in a \emph{setuid} running program and thus gain root privilege. 
    \emph{\textbf{Kernel Isolation.}}  
    These attacks~\cite{seaborn2015exploiting, qiao2016new, aweke2016anvil, van2016drammer} modify page tables entries (PTEs) to gain kernel privilege through different attack vectors. Both Seaborn and Qiao~\cite{seaborn2015exploiting, qiao2016new} utilize specific x86 CPU instructions, i.e., \emph{clflush} and \emph{movnti} respectively while Aweke et al.~\cite{aweke2016anvil} construct a specific memory-access pattern to avoid reading from the caches. Drammer~\cite{van2016drammer} aims at the ARM architecture.  
    \emph{\textbf{Virtual Machine (VM) Isolation.}} A VM owner can completely control a target VM that is within the same host by the way of page deduplication~\cite{razavi2016flip} or page-table manipulation~\cite{xiao2016one}.
    \emph{\textbf{Hypervisor Isolation.}} A VM owner can also gain the privilege of hypervisor by inducing bit-flips in PTEs~\cite{xiao2016one}.


Based on their code template that use x86 \emph{clflush} instruction to explicitly flush cache, Seaborn et al.~\cite{seaborn2015exploiting} continued the research and demonstrated the NaCI sandbox escape and kernel-privilege escalation. In the first attack, they filled available memory with authentication code and randomly picked up pairs of addresses to rowhammer the code. In the second attack, with the knowledge of pagemap and DRAM address mapping~\cite{seaborndram}, they . By doing so, efficient rowhammering can be conducted.


Bhattacharya et al.~\cite{bhattacharya2016curious}  \emph{prime+probe}~\cite{percival2005cache, osvik2006cache} and double-sided rowhammer attack to induce bit flips in memory where RSA keys are stored. 

??? Gruss et al.~\cite{gruss2016rowhammer} memory spraying launched memory 
demonstrated that rowhammer can be launched from JavaScript. Specifically, they were able to launch an attack against the page tables in a recent Firefox version.

??? Bosman et al.~\cite{bosman2016dedup} extended this work by exploiting the page deduplication feature. windows 10 also launched from JavaScript, gain arbitrary read/write access within a browser. 

??? Razvi et al.~\cite{razavi2016flip} also exploits page deduplication and rowhammer attack to attack a co-located VM and obtain its private keys.

In a paravirtual cloud, Xiao et al.~\cite{xiao2016one} had the access to \emph{pagemap} reverse-engineered DRAM address mapping, sprayed page tables, inside which bit flips were induced. 

??? Van et al.~\cite{van2016drammer} utilized the memory grooming technique to surgically place page tables onto vulnerable DRAM rows by . DMA buffer without the \emph{pagemap}. 

The known approaches to
solve this challenge are spraying, i.e., filling the entire memory
with copies of the page, or grooming, i.e., allocating the target
page in exactly the right moment

%The first general software-only defense, named ANVIL~\cite{aweke2016anvil} observes that all rowhammer attacks require unusual high memory accesses to the same DRAM rows and thus monitors specified hardware performance counters to detect such behaviors. 
%Unfortunately, the latest attack~\cite{gruss2017another} abuses Intel SGX~\cite{costan2016intel} to hide its memory-access pattern. Further, with other techniques, it can evade all the countermeasures above. 
Cross-VM Row-Hammer Attacks~\cite{xiao2016one} are demonstrated to break Xen memory isolation enforced by paravirtualized Xen and gain 

cross-VM settings,
in which a malicious VM exploits bit flips induced
by row hammer attacks to crack memory isolation enforced
by virtualization. 
exhaustively hammer a large fraction of physical
memory from a guest VM (to collect exploitable
vulnerable bits), and innovative approaches to break
Xen paravirtualized memory isolation (to access arbitrary
physical memory of the shared machine).

\cite{razavi2016flip,qiao2016new,bosman2016dedup,gruss2016rowhammer,brasser17can,seaborn2015exploiting}
}

\eat{
\zhi{it has three other disadvantages: 1. it requires CPU to feature Intel SGX~\cite{costan2016intel, mckeen2013innovative} while our attack does not need any special hardware features. 2. there are false negatives when it is determining whether a target page is at the expected physical memory location. (address-translation) 3. a single process exhausts page cache pages, which is easily detected by the OS administrator.}
}

%\subsection{Rowhammer Attacks}
We first review how rowhammer attacks achieve the different requirements, specifically, how the CPU cache is flushed, how the row buffer is cleared, and how the aggressor and victim rows are placed. 
%identify three challenges to launch a successful rowhammer attack. 
%the following challenges are identified to launch a successful double-sided hammer: (i) virtual to physical addresses mapping and physical address to DRAM mapping are necessary to make sure a pair of virtual addresses are in different rows within the same bank; (ii) CPU cache and DRAM row buffer should be bypassed to enable direct memory accesses to different rows; (iii) security-sensitive data are required to be placed onto the victim row for subsequent rowhammering. 

\mypara{Bypass CPU cache}
since frequent and direct memory access is a prerequisite for hammering,  a simple solution is to use the  \texttt{clflush} instruction for explicit CPU cache flush~\cite{kim2014flipping, seaborn2015exploiting}. 
This instruction can flush cache entries related to a specific virtual address, and thus subsequent read to the address will be served directly from the memory. \texttt{clflush}  is included in the instruction set for a process to fetch the updated data from the memory instead of the obsolete cached ones. It can be executed by an unprivileged process. It has been proposed to prohibit user processes to execute the instruction as a defense against rowhammer attacks~\cite{seaborn2015exploiting}. 
However, Qiao et al.~\cite{qiao2016new} reported that commonly used x86 instructions such as \texttt{movnti} and \texttt{movntdqa} actually bypass the CPU cache and access the memory directly. 
Moreover, carefully crafted memory-access patterns~\cite{aweke2016anvil,bhattacharya2016curious,gruss2016rowhammer,bosman2016dedup,frigo2018grand} can cause cache conflict and effectively evict the cache of the target address. This approach is particularly useful for the scripting environments where cache-related instructions are not directly available. 
At last, DMA-based memory is uncached by the CPU cache and thus it is exploited by multiple attacks~\cite{tatar2018throwhammer,lipp2018nethammer,van2018guardion,van2016drammer} to directly reach DRAM. 


\mypara{Clear row buffer}  
besides flushing the cache, rowhammer attacks also need to clear the row buffer in order to keep ``opening'' a row. Different rowhammer attacks have achieved this goal with various techniques.

Double-sided hammering performs alternate reads on different rows in the same bank. Therefore, it requires the virtual-to-physical and physical-to-hardware mappings in order to position the aggressor and victim rows. The \texttt{pagemap} provides complete information of the first mapping, but it is not accessible to the unprivileged process now. Although huge page on x86~\cite{seaborn2015exploiting} and the DMA buffers on the ARM architecture~\cite{van2016drammer} only give the partial information about the virtual-to-physical address mapping, they ensure that two virtually-continuous addresses are also physically continuous. They can also be used by rowhammer attacks. Alternatively, Glitch~\cite{frigo2018grand} relies on precise GPU-based timers to detect physically-contiguous memory. For the second mapping, AMD provides the details in their manual, and the mapping for various Intel CPUs has been reverse engineered~\cite{xiao2016one,pessl2016drama}. 

In contrast, single-sided hammering~\cite{seaborn2015exploiting} and one-location hammering~\cite{gruss2017another} do not need both mappings to clear the row buffer. To this end, single-sided hammering randomly selects multiple virtual addresses to access and it is likely that these addresses are in different rows within the same bank, thus clearing the row buffer.
{For one-location hammering, it keeps opening one randomly chose row and leverages the advanced DRAM controller to close the row. Both single-sided and one-location hammering hammer a row in a less frequent way than that of double-sided hammering, thus they are less efficient in inducing bit flips.}


\mypara{Place target objects}
the last requirement of rowhammer attacks is to manipulate the security domain into placing a security-sensitive object in a vulnerable row. This can be achieved through page-table spraying~\cite{seaborn2015exploiting,gruss2016rowhammer}, page deduplication~\cite{bosman2016dedup,razavi2016flip}, Phys Feng Shui~\cite{van2016drammer}, RAMpage~\cite{van2018guardion} and Throwhammer~\cite{tatar2018throwhammer}. However, they all require exhausting the memory in order to place the target page in the vulnerable row. 
%forced the kernel to allocate too much memory, making the target page land on the right location. 
%filled memory with copies of generated page tables, causing the kernel to place page tables onto s. 
Instead of depleting the system memory, memory waylay~\cite{gruss2017another} exhausts the page cache to influence the physical location of a target page. Without exhausting either memory or page cache, Glitch~\cite{frigo2018grand} and our memory-ambush technique can satisfy this requirement with a much constrained amount of memory but Glitch only gains the browser privilege.

\subsection{Rowhammer Defenses}
Both hardware and software defense against rowhammer attacks have been proposed. 
Hardware defenses can be based on the firmware or new hardware designs. For example, computer manufacturers, such as HP~\cite{HP}, Lenovo~\cite{LENOVO} and Apple~\cite{apple}, propose to double the refresh rate of DRAM from 64ms to 32ms. This slightly raises the bar for the attack but has been proven to be ineffective~\cite{aweke2016anvil}.
Intel suggests to use Error Correcting Code (ECC) memory to catch and correct single-bit errors on-the-fly, thus alleviating bit flips by rowhammer attacks~\cite{intelecc}. Typically, ECC can correct single-bit errors and detect double-bit errors (e.g., SECDED). However, ECC cannot prevent multiple bit errors and normally is only available on the server systems.
Probabilistic adjacent row activation (PARA)~\cite{kim2014flipping} activates/refreshes adjacent rows with a high probability when the aggressor rows are hammered many times. This could be effective but needs changes of the memory controller. 
For future DRAM architectures, new DDR4 modules~\cite{DDR4} and LPDDR4 specification~\cite{lpDDR4} propose a targeted row refresh (TRR) capability to mitigate rowhammer attacks. However, Nethammer~\cite{lipp2018nethammer} presented a network-based rowhammer attack in the face of TRR, causing kernel crashes.  
%~\zhi{never call others' defense ad-hoc or similar words}

Many software-based defenses have also been proposed. Some defenses aim to preventing attacks from misusing specific system features.  For example, researchers and developers have worked to prevent the {\tt pagemap}~\cite{shutemovpagemap,seaborn2015exploiting}, page deduplication~\cite{pagededuplication}, specific x86 CPU instructions~\cite{seaborn2015exploiting}, GPU timers~\cite{glitch}, ION contiguous heap~\cite{ION}  and memory/page-cache exhaustion~\cite{gruss2016rowhammer,van2016drammer, gruss2017another} from being abused by unprivileged attackers. 
ANVIL~\cite{aweke2016anvil} is the first system to detect rowhammer behaviors using the Intel hardware performance counters~\cite{intelOp}. However, ANVIL incurs a high performance overhead in its worst case and has false positives~\cite{brasser17can}. 
Brasser et al.~\cite{brasser2016can} patch an open-source bootloader and disable the vulnerable memory modules. Although this approach effectively eliminates all the rowhammer
vulnerabilities for legacy systems, it is not practical when most memory is susceptible to rowhammer and this method is not compatible with Windows. 

Inspired by the CATT concept, there
are other three software-only techniques achieving orthogonal instances of the physical domain isolation, that is, GuardION~\cite{van2018guardion} physically isolated DMA memory. ALIS~\cite{tatar2018throwhammer} presented physical memory isolation for network relevant memory while RIP-RH~\cite{bock2019rip} enforced physical memory isolation for target user processes. We believe that such defense techniques based on the CATT concept are also not
secure if their deployment in real-world don't carefully consider the performance design of modern OSes (i.e., they can be identified to have a similar memory-ownership issue).


